Cosmological Backgrounds of Gravitational Waves

Gravitational waves (GWs) have a great potential to probe cosmology. We review early universe sources that can lead to cosmological backgrounds of GWs. We begin by presenting definitions of GWs in flat space-time and in a cosmological setting, and discussing the reasons why GW backgrounds from the early universe are of a stochastic nature. We recap current observational constraints on stochastic backgrounds, and discuss some of the characteristics of present and future GW detectors including advanced LIGO, advanced Virgo, the Einstein Telescope, KAGRA, LISA. We then review in detail early universe GW generation mechanisms proposed in the literature, as well as the properties of the GW backgrounds they give rise to. We classify the backgrounds in five categories: GWs from quantum vacuum fluctuations during standard slow-roll inflation, GWs from processes that operate within extensions of the standard inflationary paradigm, GWs from post-inflationary preheating and related non-perturbative phenomena, GWs from first order phase transitions (related or not to the electroweak symmetry breaking), and GWs from topological defects, in particular from cosmic strings. The phenomenology of early universe processes that can generate a stochastic background of GWs is extremely rich, and some backgrounds are within the reach of near-future GW detectors. A future detection of any of these backgrounds will provide crucial information on the underlying high energy theory describing the early universe, probing energy scales well beyond the reach of particle accelerators.

==> PartProdInf.tex <==
%!TEX root = RevV.tex
Gravitational waves can be emitted classically during inflation if a tensor anisotropic stress is present during the inflationary stage. If such is the case, GWs produced inside the horizon during inflation are diluted by the exponential expansion of the background. Only once a given wavelength crosses outside the Hubble radius, does the GW amplitude remains constant. Therefore, in order to minimize the amount of dilution and provide an interesting GW signal, mechanisms of GW generation by a non-zero anisotropic stress must operate sufficiently close to the Hubble scale. 

The emission of GWs by particle production during inflation pertains to this category of GW generation processes. Several models of particle production have been discussed in the literature. In general, particle production during inflation is possible because, as the inflaton rolls down its potential, it provides a time-dependent background that carries the energy necessary for the production of sufficiently light species~\cite{Chung:1999ve}. The energy momentum tensor of the produced species acts as a non-zero anisotropic stress over the background energy-momentum tensor, hence sourcing GWs. In the following we consider two cases, differentiated by the transient and sustainable nature of the particle production mechanism.\\

{\it Transient Particle Production--.} Let us consider, for instance, a scalar field $\chi$ coupled to the inflaton $\phi$, with Lagrangian $-\mathcal{L}_\chi = (\partial \chi)^2/2 + g^2(\phi-\phi_0)^2\chi^2/2$. Analogously, we can also consider some fermion field coupled to the inflaton, with Lagrangian $-\mathcal{L}_\psi = \bar\psi\gamma^\mu\partial_\mu\psi + g(\phi-\phi_0)\bar\psi\psi$. We can also consider the dynamics of a gauge field $A_\mu$ obeying the Lagrangian $\mathcal{L} = -{1\over4}F_{\mu\nu}F^{\mu\nu}-|(\partial_\mu-gA_\mu)\Phi)|^2-V(\Phi^\dag\Phi)$~\cite{Finelli:2000sh,Cook:2011hg}, where $F_{\mu \nu} = \partial_\mu A_\nu - \partial_\nu A_\mu$ is the field strength, and $\Phi=\phi e^{i\theta}$ is a complex field. In the latter case, even though $\phi$ is not identified with the inflaton\footnote{To simplify the discussion on the particle production of the three cases (scalar $\chi$, fermion $\psi$ and vector $A_\mu$ fields), we maintain the same notation $\phi$ for the field causing the particle production, independently of the nature of the field causing the particle excitation.}, we assume it evolves during inflation in such a way that its amplitude vanishes at some point $\phi(t_0) \equiv \phi_0 = 0$. In either of the three scenarios, when $\phi$ crosses around $\phi_0$ ($\phi_0 \neq 0$ if $\phi$ is the inflaton, $\phi_0 = 0$ otherwise), the mass $m = g(\phi(t)-\phi_0)$ vanishes exactly at $t = t_0$ when $\phi(t_0) = \phi_0$. For a short period of time $\Delta t_{\rm na}$ around $t_0$, %$(t_0-\Delta t_{\rm na},t_0+\Delta t_{\rm na})$, 
\begin{eqnarray}
\Delta t_{\rm na} \sim 1/\mu\,,~~~~~~\mu^2 \equiv g\dot\phi_0\,,
\end{eqnarray}
the mass changes non-adiabatically as $\dot m \gg m^2$, leading to an explosive production of particles\footnote{$\Delta t_{\rm na}$ must be shorter than a Hubble time in order for the particle production to be efficient, i.e.~$\Delta t_{\rm na} \ll 1/H$. This implies a coupling range $g^2 \gg H^2/|\dot\phi|$.}~\cite{Kofman:1997yn}. The occupation number of the quanta created is actually independent of the spin of excited species (given the Lagrangians considered above), and it reads $n_k = {\rm Exp}\lbrace -\pi(k/\mu)^2\rbrace$~\cite{Barnaby:2012xt}. This shows clearly that only long wave modes $k \ll \mu$ are excited, as short modes evolve adiabatically around $t_0$. 

In all three cases (scalars, fermions, and vectors), GWs are generated by the anisotropic distribution of the excited species. Since particle production happens around the precise time $t_0$ when $\phi(t_0) = \phi_0$, the spectrum of GWs shows a feature at the frequency today corresponding to that moment. This feature represents an additional contribution on top of the standard irreducible vacuum tensor spectrum. 

Notably, even though the field structure of the energy-momentum tensor sourcing the GWs depends on the spin, {\it Barnaby et al}~\cite{Barnaby:2012xt} has shown that the GW produced by the excited particles is essentially independent of the spin, modulo normalization factors of order $\mathcal{O}(1)$. Let us write the total power spectrum as $\mathcal{P}_h^{\rm (tot)}(k) = \mathcal{P}_h^{\rm (vac)}(k) + \mathcal{P}_h^{\rm (s)}(k)$, with $\mathcal{P}_h^{\rm (vac)}(k) \equiv (2/\pi^2)(H/m_{\rm Pl})^2$ the vacuum contribution given by Eq.~(\ref{eq:Deltah2Prim}). Detailed calculations~\cite{Cook:2011hg,Carney:2012pk,Barnaby:2012xt} show that the contribution $\mathcal{P}_h^{\rm (s)}(k)$ from the newly created particles, distorts the total tensor power spectrum like
\begin{eqnarray}\label{eq:GWtransient}
{\Delta \mathcal{P}\over \mathcal{P}} \equiv {\mathcal{P}_h^{\rm (tot)}-\mathcal{P}_h^{\rm (vac)}\over \mathcal{P}_h^{\rm (vac)}} \equiv {\mathcal{P}_h^{\rm (s)}\over \mathcal{P}_h^{\rm (vac)}} \sim few\times\mathcal{O}(10^{-4}){H^2\over m_{\rm Pl}^2}W(k\tau_0)\left({\mu\over H}\right)^{3}\ln^2(\mu/H)\,,
%{2\over\pi^2}{H^2\over m_{\rm pl}^2}\left(1 + \alpha_s\left({\mu\over H}\right)^{p_s}W_s(k\tau_0){H_k^2\over m_{\rm pl}^2}\right) 
\end{eqnarray}
where the exact amplitude factor depends on the spin case, and $W(x) \equiv {(\sin(x)-x\cos(x))^2\over x^3}$. This correspond to a scale-dependent distortion which reaches its biggest amplitude around the horizon scale $x_0 = k\tau_0 \simeq 1$, with $W(x_0) \simeq 0.5$ (note that in this section the conformal time is denoted $\tau$). The maximum distortion of the vacuum tensor spectrum is then obtained around the Hubble scale at the moment of particle production $t_0$. When the excited species are either a scalar field or a fermion field, $\phi$ is the inflaton, so we can use Eq.~(\ref{eq:DeltaR2}) to derive the relations $H^2/m_{\rm Pl}^2 \simeq 8\pi^2\epsilon \mathcal{P}_{\mathcal{R}}$ and $\mu/H = (g/2\pi)^{1/2}/\mathcal{P}_{\mathcal{R}}^{1/4}$. Plugging these into Eq.~(\ref{eq:GWtransient}), we find the maximum distortion as $\Delta\mathcal{P}/\mathcal{P} \sim \epsilon\mathcal{O}(10^{-2})\mathcal{P}_{\mathcal{R}}^{1/4}(g/2\pi)^{3/2}\left(\ln\left(g\over 2\pi\right) - {1\over2}\ln(\mathcal{P}_{\mathcal{R}})\right)^2$. Using CMB measurements, we know that $\epsilon < 0.0068$ and $\mathcal{P}_{\mathcal{R}} \simeq 2.2\cdot 10^{-9}$. Plugging in these numbers, we see that the new contribution represents a negligible distorsion $\Delta\mathcal{P}/\mathcal{P} \ll 1$ at the CMB scales, of the otherwise quasiscale invariant quantum fluctuations background. Assuming that the inflaton is in slow-roll all the way from the exit of the CMB scales till the end of inflation, we conclude that this distortion is always negligible, even if the particle production takes place towards the end of inflation when $\epsilon$ approaches unity\footnote{It is interesting to note that if the scalar perturbations were much larger at smaller scales than at CMB scales, i.e.~$\mathcal{P}_{\mathcal{R}} \gg 10^{-9}$ at the scales leaving the Hubble radius towards the end of inflation, we might expect then to reach a non-negligible distortion $\Delta\mathcal{P}/\mathcal{P} \gtrsim \mathcal{O}(1)$. However this requires a specific somehow contrived set up, demanding not only particle production at the right moment towards the end of inflation, but also some feature in the inflaton potential creating large curvature perturbations just at small scales.}.

Note that if there are several occurrences of particle production, like for example in the model of Ref.~\cite{Green:2009ds}, the sourced GW add up and the resulting GW spectrum can become scale invariant. However, even in this case, it is largely subdominant with respect to the inflationary tensor spectrum and cannot be detected in the CMB~\cite{Cook:2011hg}. It seems that in these scenarios, we cannot obtain observationally interesting signatures in the GW background. The GW sourced in this model are much smaller than the scalar perturbations, since the quanta of the species excited are non-relativistic when they are produced, and therefore their quadrupole moment is highly suppressed. Imposing that the scalar curvature spectrum satisfies the observational constraints (i.e.~no bump has been observed by CMB measurements) reduces the amplitude of the GW feature down to a further irrelevant level. Ref.~\cite{Barnaby:2012xt} remarks that only a sufficiently high amplification of the GW signal in a model with multiple bursts of particle production could produce a GW signal observable in the CMB; however, such a model is not identified yet.

To work out the tensor spectrum distortion in the case of a gauge field excitation, we must determine first the nature of the field $\phi$, and thus its velocity $\dot\phi_0$. Gauge invariance requires the potential $V(\Phi)$ to be a function of $|\Phi|^2$, and hence $\Phi = 0$ to be either a maximum or a minimum of $V(\Phi)$, so that $V'(\Phi = 0) = 0$. We conclude that $\Phi$ cannot be in a slow-roll regime, as otherwise the velocity $\dot\Phi \propto V'(|phi)$ would vanish. The field $\Phi$ must be therefore fast rolling. A simple set up consist then in assuming that $\Phi$ has a super-Hubble mass $m_{\Phi} \gg H$, and a large amplitude $\Phi_i$ (acquired at some early stage during inflation). Under these circumstances, the field $\Phi$ oscillates many times per Hubble time, and the (absolute value of the) velocity when crossing around zero is given by $\dot\phi_0 \sim m_{\Phi}\Phi_i$. Requiring that the energy of $\Phi$ is sub-dominant versus the inflaton energy, implies that $\gamma \equiv m_{\Phi}^2\Phi_i^2/6H^2m_{\rm Pl}^2 \ll 1$. This implies that, up to a logarithmic correction, $\Delta\mathcal{P}/\mathcal{P} \sim \mathcal{O}(10^{-4})g^{3/2}(H/m_p)^{1/2} \ll 1$, rendering again this signal as insignificant.\\

%so we can express its velocity using the slow-roll condition $|\dot\phi_0| \simeq \sqrt{2\epsilon}Hm_{\rm Pl}$, where $\epsilon \ll 1$. Therefore $\Delta\mathcal{P}/\mathcal{P} \sim \mathcal{O}(10^{-4}) \epsilon^{3/4} g^{3/2}(H/m_p)^{1/2}\left(\ln(g\epsilon^{1/2}) + \ln(m_p/H)\right)^2$, 
%
 

%with the different powers $p_s = 3, 5, 7$ corresponding to a spin $s = 0, {1\over2}, 1$, respectively, depending on whether the excited field was a scalar, a fermion, or a gauge boson. 
 
%In the case of a fermion $\psi$, a similar calculation leads to $\Delta\mathcal{P}_h/\mathcal{P}_h \sim \mathcal{O}(10^{-4})\epsilon^{5/4}g^{5/2}(m_p/H)^{1/2}$. $A priori$ it is unclear whether this contribution is necessarily smaller than unity. Let us maximize the possible effect, considering that the fermion production takes place well after CMB scales left the Hubble radius, so that we can take a slow-roll parameter larger than its CMB upper bound, say $\epsilon \sim 0.1$. %\footnote{Let us note that in ordinary chaotic inflation, stability of the inflaton potential under radiative corrections, requires $g \lesssim 10^{-3}$. However, in order to maximize $\Delta \mathcal{P}/\mathcal{P}$, we will require a much smaller Hubble rate than for for chaotic inflation models, we for the shake of the argument, we shall consider a hypothetical scenario different than Chaotic inflation and where we somehow manage to have $g^2$ without spoiling inflation.} 
%To maximize $\Delta\mathcal{P}/\mathcal{P}$, let us also take $g = 10^{-3}$, which corresponds to the maximum value for the coupling strength which does not to spoil the flatness of the inflaton potential due to radiative corrections. Under these assumptions, in order to obtain $\Delta\mathcal{P}/\mathcal{P} \gtrsim 1$, we still need $H \lesssim 5\cdot 10^{-7}m_{\rm Pl}$. The current upper bound on $H$ at the CMB scales is $H \lesssim \cdot 10^{14}$ GeV $\simeq 10^{-5}m_{\rm Pl}$. Given the upper bound on the amplitude today of the vacuum contribution $\Omega_{\rm GW}^{\rm (vac)} \leq 5\cdot 10^{-16}$, and the fact that such signal scales as $\Omega_{\rm GW}^{\rm (vac)} \propto (H/m_{\rm Pl})^2$, we arrive at the following conclusion: a distortion of $\mathcal{O}(1)$ of the GW background created by vacuum fluctuations, can only be attained if the total background has an amplitude today of the order of $\Omega_{\rm GW} \sim 10^{-18}$. This represents a very tiny signal, not accessible to any planned GW detector. For Hubble rates smaller than $H \lesssim 5\cdot 10^{-7}m_{\rm Pl}$, the distortion of the vacuum signal will be larger than $\mathcal{O}(1)$, so the total signal will be dominated by the sourced contribution $\mathcal{P}_h^{\rm (tot)} \simeq \mathcal{P}_h^{\rm (s)}$. However, the latter signal scales as $\mathcal{P}_h^{\rm (s)} \propto (H/m_{\rm Pl})^{3/2}$, so decreasing further $H$ will only render its amplitude smaller and smaller.

%However, the amount of GWs induced by vectors $A_\mu$ equals, per helicity mode, that induced by scalars $\chi$, and it is therefore negligible \cite{Cook:2011hg}. This model has been recently reanalised in Ref.~\cite{Barnaby:2012xt}, which derives also the scalar curvature spectrum and bispectrum produced by the vector field. As for the tensors, they all show a bump feature for scales leaving the horizon at the moment when the gauge fields are produced, i.e. when their mass crosses zero during the evolution of $\psi(t)$.


{\it Sustainable Particle Production --.} A more promising scenario of particle production, which can give rise to observable GW, consist in introducing a derivative coupling between the inflaton and a gauge field~\cite{Barnaby:2010vf}. In this case, the gauge field can remain massless as the inflaton rolls down its potential, and particle production can happen continuously throughout inflation. This occurs in particular when the inflaton $\phi$ couples to a gauge field through an interaction term of the form 
%
\begin{eqnarray}\label{eq:phiFF}
\Delta{\cal L}=-\frac{1}{4\,\Lambda}\,\phi\,F_{\mu\nu}\,\tilde{F}^{\mu\nu}\,,
\end{eqnarray}
with $F_{\mu \nu}$ the field strength and $\tilde{F}_{\mu \nu} \equiv {1\over 2}\epsilon_{\mu\nu\alpha\beta}F^{\alpha\beta}$ its dual, whereas $\Lambda$ is a (dimension-full) coupling controlling the interaction between the inflaton and the gauge field. Such an interaction is natural in models where the inflaton field is a pseudoscalar. These models have received a significant amount of interest in the literature\cite{Freese:1990rb,Senatore:2011sp,Pajer:2013fsa,MORE!!}, due to, a) their radiative stability, and b) the interesting phenomenology they can generate. Radiative stability plays in fact a crucial role in the construction of inflationary models, helping to discriminate between technically natural potentials (for which quantum properties of the theory are under control), and models which require some parameter fine tuning one way or another (for which the UV part of the theory is unresolved). Ensuring radiative stability can be easily done by assuming a (softly broken) {\em shift symmetry}, i.e.~an invariance of the theory under the transformation $\phi\to\phi+\phi_0$, $\phi_0$ being an arbitrary constant. One of the very few operators of low dimension that are allowed by an exact shift symmetry is precisely the interaction Eq.~(\ref{eq:phiFF}), expected to be generated in a large of class of technically natural models of inflation. 

An interaction like Eq.~(\ref{eq:phiFF}) generates a very rich phenomenology. The equation of motion of the (conformaly transformed) $\pm 1$-helicity modes $A_\pm({\bf k},\,\tau)$ of the gauge field reads~\cite{Anber:2006xt} 
%
\begin{eqnarray}\label{eq:XiParam}
\frac{d^2A_\pm({\bf k},\,\tau)}{d\tau^2}+\left[k^2\pm 2\,\xi\,\frac{k}{\tau}\right]\,A_\pm({\bf k},\,\tau)=0\,,~~~~
\xi\equiv\frac{\dot\phi}{2\,f\,H}\,,
\end{eqnarray}
%
with $\tau$ the conformal time, but $\dot\phi$ the time derivative of the inflaton with respect to cosmic time $t$, whilst $H$ is the Hubble parameter. The $\pm$ sign in Eq.~(\ref{eq:apm_eulerlagrange}) implies that for sufficiently long wavelengths $-k\,\tau<2\,\xi$, one (and only one) of the two helicity modes is exponentially amplified during inflation.  For constant and positive parameter $\xi > 0$, an exact solution of Eq.~(\ref{eq:XiParam}) can be found~\cite{Anber:2006xt}, showing that only $A_+$ (and not $A_{-}$) is amplified by a factor $\sim e^{\pi\,\xi}$ for\footnote{In slow-roll inflation, as long as back reaction of the gauge field into the background inflaton dynamics is negligible, $\xi \simeq \frac{M_{\rm Pl}}{\Lambda}\,\sqrt{\frac{\epsilon_\phi}{2}}$. Hence, unless $\epsilon_\phi \lll 1$, a value of $\Lambda$ within 1-2 orders of magnitude below $M_{\rm Pl}$, leads always to a value $\xi\gtrsim {\cal O}(1)$.} $\xi\gtrsim {\cal O}(1)$. The fact that only one of the photon helicities is amplified is reflects, in fact, the parity-violating nature of the operator Eq.~(\ref{eq:phiFF}). 

The exponentially excited gauge fields act in turn as a powerful source of gravitational waves (as well as of scalar perturbations). Since the energy-momentum tensor of photons is quadratic in the gauge field amplitude, the tensor (and scalar) perturbations sourced by the photons enjoy necessarily non-Gaussian statistics, having e.g.~a non zero bispectrum function (three-point expectation value). The scalar bispectrum, in particular, has an approximate equilateral shape~\cite{Barnaby:2010vf}, with a non-linear parameter of the order $f_{NL}^{\rm {equil}} \sim 10^6\,\frac{H^6}{|\dot\phi|^3}\,\frac{e^{6\,\pi\,\xi}}{\xi^9}$. The non-detection of scalar non-Gaussianities at the CMB by the Planck experiment, implies in fact a strong constraint on this scenario, with $\xi\lesssim 2.5$ at $95\%$ C.L.~\cite{Ade:2015lrj, Ade:2015ava}. As we will see shortly, see Eq.~(\ref{eq:Omega1}) below, the sourced gravitational waves for such small values of $\xi$, are unfortunately too weak to be observed.

The parameter $\xi$ is in reality a time dependent quantity, so the spectrum of photons is scale dependent. This forces automatically, the spectrum of GWs created by the photons, to be scale dependent as well. In general, the $\xi$ will increase as the inflationary stage progresses, since $|\dot\phi|$ typically increases, whilst $H$ decreases, as we approach towards the last stages of inflation. This way, we can easily consider a situation with $\xi$ being smaller than $2.5$ or so at the time when CMB scales left the horizon, but with $\xi$ growing later on, when shorter than CMB scales leave successively the horizon. This way the Planck constraints~\cite{Meerburg:2012id,Ade:2015lrj} on the power spectra and bispectra at the CMB scales can be fully satisfied, while at the same time a large GW signal can be generated at shorter scales.  The time dependence of $\xi$, and hence the scale dependence of the spectrum of GWs,  depends of course on the specific choice of inflaton potential\footnote{It also depends eventually on the back-reaction of the excited photons over the background, if the backreaction becomes large enough.}

In these models, the standard GWs from vacuum fluctuations and the additional sourced GWs created by the excited gauge fields, are statistically uncorrelated, so the total tensor power spectrum is the sum of the power spectra of these two contributions, without interference. For $\xi\gtrsim {\cal O}(1)$, a detailed calculation of the spectrum of tensor modes~\cite{Barnaby:2010vf,Sorbo:2011rz} shows that
%
\begin{eqnarray}\label{eq:pGW_sourced}
\mathcal{P}_{h}^{(tot)} \left( k \right) &\equiv & \frac{k^3}{2 \pi^2} \sum_{a=\pm} \left \vert h_{a} \left( k \right) \right \vert^2 = \mathcal{P}_{h}^{\rm (vac)}(k) + \mathcal{P}_{h}^{\rm (pp)}(k)\\
&=& \mathcal{P}_{h}^{\rm (vac)}\left(1+\Delta\mathcal{P}_{h}\right) \simeq \frac{2\,H^2}{\pi^2\,M_{\rm Pl}^2}\left(1 +  4.3 \cdot 10^{-7} \frac{H^2}{M_{\rm Pl}^2}\frac{e^{4 \pi \xi}}{\xi^6}\right) \,. 
\end{eqnarray} 
%
where $pp$ stands for particle production. Let us note that even though it is not indicated explicitly, the last expression in the $rhs$ depends on $k$, as both $H$ and $\xi$ are evaluated at the time when a given mode $k$ leaves the horizon during inflation. 

The power spectrum is related to the fractional GW energy density by $\Omega_{\rm GW} h^2 = \frac{\Omega_{\rm R,0} h^2}{24} \, P_{\rm GW}$, where $\Omega_{R,0} h^2 \equiv \rho_{{\rm R},0} h^2 / 3 H_0^2 M_{Pl}^2 \simeq 4.18 \cdot 10^{-5}$ (one needs to include also the neutrinos as if they were still relativistic today). In Fig.~\ref{fig:local-nT} we plot $h^2\Omega_{\rm GW}$ as a function of frequency, for a quadratic inflaton potential and with $\Lambda = M_{\rm Pl}/35$. We can notice three different regimes: {\em i)} dominance of the of the vacuum fluctuations contribution at large scales ($f\lesssim 10^{-5}$~Hz, {\em ii)} dominance of the sourced GWs contribution at intermediate scales ($10^{-5}$~Hz$ \lesssim f\lesssim 1$~Hz), when the back reaction of the gauge fields is still negligible (so the time-dependence of $\dot\phi$ and $H$ is determined by the standard slow-roll equations), and {\em iii)} dominance of the sourced GWs contribution at small scales ($f\gtrsim 1$~Hz), when the back reaction of the gauge fields cannot be neglected any more. Due to conservation of energy, the production of photons implies a reduction of the kinetic energy of the inflaton, so that the growth of $|\dot\phi|$ is slowed down, resulting into a flattening of $\Omega_{\rm GW}\,h^2$ at the smallest scales (highest frequencies). It is worth noticing that in the simplest slow-roll scenarios, $|\dot\phi|$ increases monotonically whereas $H$ decreases monotonically, resulting in a blue spectrum of sourced GWs. It is however possible to consider scenarios where $\xi$ has a transient behavior, resulting into a localized bump in the GW spectrum, see~\cite{Namba:2015gja,Garcia-Bellido:2016dkw}. 

While Eq.~(\ref{eq:pGW_sourced}) the amplitude of sourced GW background, it is worth noting that in these scenarios, the amplitude of the power spectrum does not characterize completely this background. There are, in fact, two very distinctive properties of the sourced background, namely its chirality and its non-Gaussian statistics, that makes it quite special:

\begin{itemize}

\item {\em Parity violation.} Eq.~(\ref{eq:pGW_sourced}) describes the total power in GWs, given by the sum of the individual contributions from left- and right-handed modes. Each of these modes are excited separately as $\mathcal{P}_{h,+}^{\rm (pp)} 8.7\cdot \cdot 10^{-8} \frac{H^4}{M_{Pl}^4}\frac{e^{4 \pi \xi}}{\xi^6}$ and $\mathcal{P}_{h,-}^{\rm (pp)} \simeq 2.1\cdot 10^{-3} \mathcal{P}_{h,+}^{\rm (pp)}$. The different amplitude between the left- and the right-handed tensor modes is a sign of the parity-violating nature of Eq.~(\ref{eq:phiFF}). Hence, the sourced GW background is highly chiral, what represents a very distinctive signature of these scenarios. For a discussion on the strategies for detecting a stochastic chiral backgrounds of GWs (with Earth-based detectors), see~\cite{Crowder:2012ik}.

\item {\em Non-Gaussianity.} As discussed, both scalar and tensor perturbations sourced by the excited gauge field obey non-Gaussian statistics. For an approximately constant $\xi$, the three point function of the GWs in this scenario was computed in~\cite{Cook:2013xea}. The shape of the bispectrum is close to equilateral, with an amplitude (evaluated in the exact equilateral configuration $|{\bf{k}}_1|=|{\bf{k}}_2|=|{\bf{k}}_3|=k$) given by $\langle \hat{h}_+({\bf{k}}_1)\,\hat{h}_+({\bf{k}}_2)\,\hat{h}_+({\bf{k}}_3)\rangle_{\rm {equil}}=6.1\times 10^{-10}\,\frac{H^6}{M_{Pl}^6}\,\frac{e^{6\pi\xi}}{\xi^9}\,\frac{\delta^{(3)}({\bf{k}}_1+{\bf{k}}_2+{\bf{k}}_3)}{k^6}$, which corresponds, approximately, to power spectrum to the power $3/2$. Constraints on the tensor bispectrum from CMB measurements~\cite{Ade:2015ava} yield a constraint on $\xi$ (on CMB scales) similar from that from the CMB scalar bispectrum measurements ~\eqref{eq:fNL}. The one-to-one correspondence of the power spectrum and bispectrum represents a unique signature of this scenario. For a discussion on the detectability of non-Gaussian primordial signatures of GWs at interferometers, see~\cite{Thrane:2013kb}. 

\end{itemize}

In summary, the mechanism of gauge field amplification from the interaction (\ref{eq:phiFF}) is extremely interesting, {\em a)} it is inherent to well motivated inflationary models, {\em b)} it naturally leads to a GW signal that grows with time during inflation, typically with a significant blue spectrum that can be probed by LISA and other upcoming experiments, hence allowing to probe the inflationary period well after the CMB scales left the horizon, {\em c)} the stochastic background of GWs produced has very characteristic properties that allow to distinguish it from other backgrounds, namely it is highly chiral, and {\em d)} it is highly non-Gaussian, with a unique relation between the three- and two-point functions of the tensor modes $k^6 B \simeq 23 P_{\rm GW}^{3/2}$.

The sourced GW signal $h^2\Omega_{\rm GW}^{\rm (pp)} \simeq 1.5 \cdot 10^{-13} \frac{H^4}{M_{\rm Pl}^4}\frac{e^{4 \pi \xi}}{\xi^6}$ (for $\xi > 1$ ) can be locally parametrized in the form $h^2\Omega_{\rm GW} \propto f^{n_T}$, by evaluating $H$ and $\xi$ as a function of the e-folding $N$ corresponding the moment when a given wavenumber $k$ left the horizon. The frequency $f = k/2 \pi$ corresponding to that wavenumber can then be related to the number of e-folds by $N = N_{\rm CMB} + {\rm ln} \frac{k_{\rm CMB}}{0.002 \, {\rm Mpc}^{-1}} -40.3 - {\rm ln } \left( \frac{f}{\rm Hz} \right) + {\rm ln } \left( \frac{H_N}{H_{\rm CMB}} \right)$ $\simeq 19.7- {\rm ln } \left( \frac{f}{\rm Hz} \right) + {\rm ln } \left( \frac{H_N}{H_{60}} \right)$, where in the second expression it was assumed that the Planck pivot scale $k_{\rm CMB} = 0.002 \, {\rm Mpc}^{-1}$ exited the horizon at $N_{\rm CMB} = 60$. At any value of the frequency we can define the spectral tilt $n_T(f) \equiv \frac{d \ln \Omega_{\rm GW} h^2 }{d \ln f}$. Detailed calculations~\cite{Bartolo:2016ami} lead to 
\begin{eqnarray}
n_T = \frac{ - 4 \epsilon + \left(4 \pi \xi - 6 \right) \left(  \epsilon - \eta \right)}{1-\epsilon} \simeq  - 4 \epsilon + \left(4 \pi \xi - 6 \right) \left(  \epsilon - \eta \right) \;, 
\label{eq:nT}
\end{eqnarray}
where the slow-roll parameters refer to $\epsilon_H$ [Eq.~(\ref{eq:eH})] and $\eta_\phi$ [Eq.~(\ref{eq:slowroll})]. In the limit of negligible back reaction from the gauge fields, one can also use $\epsilon_H \rightarrow \epsilon_V$ and $\eta_\phi \rightarrow \eta_V - \epsilon_V$, with $\epsilon_V$ and $\eta_V$ in Eq.~(\ref{eq:slowroll}) related to the inflaton potential. 

\begin{figure}[t]
\centerline{
\includegraphics[width=12.0cm]{../Figures/OmegaGW_GlobalAndLocal_NvsFreqCorr.png}
}
\caption{Numerical spectrum of GWs today $h^2\Omega_{\rm GW}$ for a model of quadratic inflaton potential, with inflaton - gauge field coupling $\Lambda =  M_{Pl} / 35$ (continuous line) versus local parametrization $h^2\Omega_{\rm GW} \propto (f/f_*)^{n_T}$, evaluated at various pivot frequencies $f_*$ and with spectral tilt $n_T$ obtained from successive approximations to the analytic expression Eq.~(\ref{eq:nT}).}
\label{fig:local-nT}
\end{figure}
For the range of $\xi$ that future detectors will be able to probe [e.g.~$\xi \gtrsim 3.5$ for LISA, see Fig.~(\ref{fig:Xi_vs_SR})], the term $-4 \epsilon$ in the final expression of Eq.~(\ref{eq:nT}) is actually negligible compared to the other terms. We can then further approximate the tilt as $n_T \simeq  \left(4 \pi \xi - 6 \right) \left( \epsilon - \eta \right)$. The advantage of this simplified tilt is that it allows to reduce the number of independent variables in which the GW signal depends on, from $\lbrace H_N,\xi,\epsilon,\eta\rbrace$ to $\lbrace H_N,\xi,(\epsilon-\eta)\rbrace$. The local parametrization allows us this way to obtain a model-independent parameter estimation based on the sensitivity curves of a given GW detector. In particular, {\it Bartolo et al} have analyzed the ability of LISA to probe the parameter space of this scenario.

For sufficiently small slow-roll parameters, $(\epsilon-\eta)\ll 0.1$, the minimum $\xi$ required for a GW signal $h^2\Omega_{\rm GW}(f)$ to be above the sensitivity curve of the (best) LISA configuration, is essentially independent of the spectral tilt $n_t$, and hence independent of the slow-roll parameters. This explains the horizontal lines marked as $\xi_{\rm min}$ in the plot. Of course, $\xi_{\rm min}$ depends on the inflationary Hubble scale $H_*$ corresponding to those frequencies. In the left panel it is also depicted, as a reference, the $(\xi,\epsilon-\eta)$ behavior for a quadratic inflation model evaluated numerically for couplings $30 \lesssim M_{Pl}/\Lambda \leq 35$. The Hubble rate in chaotic inflation with a quadratic potential at the e-fold $N_* \sim 25$ (corresponding to the frequencies a the maximum sensitivity of LISA) is $H_c \sim 2.6 \cdot 10^{-5} M_{Pl} \simeq 6.4 \cdot 10^{13}$ GeV. Taking this value as a reference, we see that LISA cannot probe any Hubble rate smaller than $\sim \mathcal{O}(10^{-2})H_c$, as a too large $\xi_{\rm min}$ is in tension with perturbativity requirements~\cite{Peloso:2016gqs}. If we take $\xi_{\rm min} = 5.5$ as the maximum tolerated value at $N_* \simeq 25$, the minimum Hubble rate that can be probed by the (best) LISA configurations is $H_{\rm min} \simeq 6.3 \cdot 10^{11}$ GeV.

\begin{figure}[t]
\begin{center}
\includegraphics[width=7.0cm]{../Figures/Xi_vs_SR_HubbleVarying_LISA_Config1.pdf}
\includegraphics[width=7.0cm]{../Figures/Xi_vs_Hubble_SR01.pdf}
\end{center}
\caption{{\it Left}: Region in the $(\xi,\epsilon-\eta)$ parameter space that LISA can probe, using the best configuration of LISA. As a reference, we also include the points corresponding to quadratic chaotic inflation for inflaton-gauge field coupling $M_{Pl}/|Lambda = 35, 34, 33, 32$ and $31$. The spectral index $n_T$ is well approximated by the simple formula $n_T\simeq (4\pi\xi-6)\,(\epsilon-\eta)$. RIght: Regions in the $\xi-H$ parameter space that LISA can probe for the best (blue region) and worst (pink region) configurations. In the left panel we show the parameter space for $(\epsilon-\eta) = 0.02$, whereas in the right panel we show it for $(\epsilon-\eta) = 0.1$.}
\label{fig:Xi_vs_SR}
\end{figure}

If the slow-roll parameters are sufficiently large, a GW signal with a peak amplitude smaller than minimum amplitude reached by the LISA best sensitivity curve, can still be observed thanks if its spectral tilt $n_T$ is sufficiently large. A scenario capable of producing such a signal becomes of course more and more contrived, the larger the slow-roll parameters. Besidesa GW background with such a large tilt requires also a mechanism to prevent any further growth of the GW amplitude at higher frequencies, otherwise this would violate the BBN bound. Thus, restricting ourselves to $(\epsilon-\eta) \leq 0.1$, the minimum tilt $n_T$ required for such a detection can be determined, and correspondingly the minimum slow-roll parameter combination $(\epsilon-\eta)_{\rm min}$ required for the amplitude of the signal to cross the LISA curve. A detailed analysis~\cite{Bartolo:2016ami} for LISA's best sensitivity curve shows that $\xi \geq \xi_{\rm min,0.1} \simeq 3.58$. We observe that for GW signals with a peak frequency below the maximum LISA sensitivity, the minimum $\xi$ required to probe the signal with LISA is slightly smaller than, but still of the order of, the asymptotic constant $\xi_{\rm min}$ values obtained for small $(\epsilon-\eta)$.

The local parametrization allows also to obtain contour regions in the $(\xi,H)$ plane of parameters, for a fixed value of $(\epsilon-\eta)$. Taking as a reference the Hubble rate $H_c \simeq 6.4\cdot 10^{13}$ GeV at the e-fold $N_* \sim 25$ corresponding to LISA detection threshold (minimum of the sensitivity curve), in the right panel we show the Hubble rate in units of $H/H_c$. If the slow-roll parameter combination is sufficiently small, say $(\epsilon-\eta) < 0.05$, we are in the asymptotic regime where $\xi > \xi_{\rm min}$ suffices to guarantee a detection by LISA (actually independently of the $(\epsilon-\eta)$ value). In the right panel we show the region of the $(\xi,H/H_c)$ parameter space compatible with a detection by LISA for $(\epsilon-\eta) \leq 0.1$. The panels shows very clearly the inability of LISA (and of any detector in general) to measure a signal for small inflationary Hubble rates, as the minimum $\xi$ required for a detection grows exponentially fast as the Hubble rate decreases. 



 




